A review of high order strong stability preserving two-derivative explicit, implicit, and IMEX methods

High order strong stability preserving (SSP) time discretizations ensure the nonlinear non-inner-product strong stability properties of spatial discretizations suited for the stable simulation of hyperbolic PDEs. Over the past decade multiderivative time-stepping have been used for the time-evolution hyperbolic PDEs, so that the strong stability properties of these methods have become increasingly relevant. In this work we review sufficient conditions for a two-derivative multistage method to preserve the strong stability properties of spatial discretizations in a forward Euler and different conditions on the second derivative. In particular we present the SSP theory for explicit and implicit two-derivative Runge--Kutta schemes, and discuss a special condition on the second derivative under which these implicit methods may be unconditionally SSP. This condition is then used in the context of implicit-explicit (IMEX) multi-derivative Runge--Kutta schemes, where the time-step restriction is independent of the stiff term. Finally, we present the SSP theory for implicit-explicit (IMEX) multi-derivative general linear methods, and some novel second and third order methods where the time-step restriction is independent of the stiff term.

==> command_file.tex <==
\newcommand{\Aep}{A^{\epsilon} }
\newcommand{\bep}{b^{\epsilon} }
\newcommand{\cep}{c^{\epsilon}}
\newcommand{\Fep}{F^{\epsilon} }
\newcommand{\Ahat}{\widehat{A} }
\newcommand{\bhat}{\widehat{\vb} }
\newcommand{\Chat}{\widehat{\vc} }
\newcommand{\Adot}{\dot{A} }
\newcommand{\bdot}{\dot{\vb}}
\newcommand{\Cdot}{\dot{\vc}}
\newcommand{\qh}{\hat{q}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bq}{\mathbf{q}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\br}{\mathbf{r}}
\newcommand{\imh}{{i-\frac{1}{2}}}
\newcommand{\iph}{{i+\frac{1}{2}}}
\newcommand{\ipmh}{{i \pm \frac{1}{2}}}
\newcommand{\jph}{{j+\frac{1}{2}}}
\newcommand{\Aop}{{\cal A}}
\newcommand{\Bop}{{\cal B}}
\newcommand{\Wop}{{\cal W}}
\newcommand{\Oop}{{\cal O}}
\newcommand{\DQ}{\Delta Q}
\newcommand{\Dq}{\Delta q}
\newcommand{\Dx}{\Delta x}
\newcommand{\Dy}{\Delta y}
\newcommand{\Du}{\Delta u}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\Lop}{{\cal L}}
\newcommand{\Sop}{{\cal S}}
\newcommand{\Fop}{{\cal F}}
\newcommand{\Dofr}{{\cal D}(r)}
\newcommand{\Dt}{\Delta t}
\newcommand{\bbA}{\mathbf{A}}
\newcommand{\bbZ}{\mathbf{Z}}
\newcommand{\bbK}{\mathbf{K}}
\newcommand{\bbI}{\mathbf{I}}
\newcommand{\bbb}{\bar{\mathbf{b}}}
\newcommand{\bbe}{\mathbf{e}}
\newcommand{\bbone}{\mathbf{1}}
\newcommand{\lnorm}{\left\|}
\newcommand{\rnorm}{\right\|}
\newcommand{\cR}{{\cal R}}
\newcommand{\dx}{\Delta x}
\newcommand{\dt}{\Delta t}
\newcommand{\aij}{\alpha_{i,j}}
\newcommand{\bij}{\beta_{i,j}}
\newcommand{\lt}{\tilde{L}}

\newcommand{\hf}{\frac{1}{2}}
\def\half{\frac{1}{2}}
\newcommand{\fracStrut}{\rule[-1.0ex]{0pt}{3.1ex}}
\newcommand{\hfs}{\ensuremath{\frac{1}{2}}\fracStrut}
\newcommand{\scinot}[2]{\ensuremath{#1\times10^{#2}}}
\newcommand{\dee}{\mathrm{d}}
\newcommand{\dye}{\partial}
\newcommand{\diff}[2]{\frac{\dee #1}{\dee #2}}
\newcommand{\pdiff}[2]{\frac{\dye #1}{\dye #2}}
\newcommand{\Real}{\mathbb{R}}
\newcommand{\Complex}{\mathbb{C}}
% matrices
\newcommand{\m}[1]{\mathbf{#1}}
\newcommand{\my}{\m{y}}
\newcommand{\mR}{\m{R}}
\newcommand{\mP}{\m{P}}
\newcommand{\mW}{\m{W}}
\newcommand{\mQ}{\m{Q}}
\newcommand{\mD}{\m{D}}
\newcommand{\mDdot}{\m{\dot{D}}}
\newcommand{\mAdot}{\m{\dot{A}}}
\newcommand{\mA}{\m{A}}
\newcommand{\mAh}{\m{\hat{A}}}
%\newcommand{\mSdot}{\m{\dot{S}}}
\newcommand{\mS}{\m{S}}
%\newcommand{\mSh}{\m{\hat{S}}
%\newcommand{\mzero}{\m{0}}
% these use the upgreek package to get non-italic greek, which doesn't
% seem to work with \mathbf so these have to be setup manually to
% match \m

\newcommand{\matalpha}{\boldsymbol{\upalpha}}
\newcommand{\matbeta}{\boldsymbol{\upbeta}}
\newcommand{\mattheta}{\boldsymbol{\uptheta}}
\newcommand{\mateta}{\boldsymbol{\upeta}}
\newcommand{\matmu}{\boldsymbol{\upmu}}
\newcommand{\matlambda}{\boldsymbol{\uplambda}}
\newcommand{\matgamma}{\boldsymbol{\upgamma}}
\newcommand{\matdelta}{\boldsymbol{\updelta}}
% vectors
\renewcommand{\v}[1]{\boldsymbol{#1}}
\newcommand{\transpose}{^\mathrm{T}}
\newcommand{\thT}{\mattheta\transpose}
\newcommand{\bT}{\v{b}\transpose}
\newcommand{\bh}{\hat{b}}
\newcommand{\vbh}{\hat{\v{b}}}
\newcommand{\bhT}{\hat{\v{b}}\transpose}
\newcommand{\vb}{\v{b}}
\newcommand{\vc}{\v{c}}
\newcommand{\vP}{\v{P}}
\newcommand{\ve}{\v{e}}
\newcommand{\vu}{\v{u}}
\newcommand{\vl}{\boldsymbol{l}}
\newcommand{\vv}{\v{v}}
\newcommand{\vx}{\v{x}}
\newcommand{\vy}{\v{y}}
\newcommand{\vd}{\v{d}}
\newcommand{\va}{\v{a}}
\newcommand{\vf}{\v{f}}
\newcommand{\vt}{\v{t}}
\newcommand{\vT}{\v{T}}
\newcommand{\Matlab}{{\sc Matlab}\xspace}
\newcommand{\BARON}{{\sc Baron}\xspace}
\newcommand{\code}[1]{\textsf{#1}}
% the SSP coefficient
\newcommand{\sspcoef}{\mathcal{C}}
\newcommand{\clin}{\sspcoef_{\textup{lin}}}
\newcommand{\ceff}{\sspcoef_{\textup{eff}}}
\newcommand{\DtFE}{\Dt_{\textup{FE}}}
\newcommand{\tDtFE}{\tilde{\Dt}_{\textup{FE}}}
\newcommand{\Inc}{\textrm{Inc}}

\newcommand{\dF}{\dot{F}}
\newcommand{\ty}{\tilde{y}}
\newcommand{\tu}{\tilde{u}}
\newcommand{\pt}{\tilde{p}}
\newcommand{\lte}{\tau}
\newcommand{\ste}{\boldsymbol{\tau}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\bty}{\mathbf{\ty}}
\newcommand{\btu}{\mathbf{\tilde{u}}}

\newcommand{\gerr}{\epsilon}
\newcommand{\gserr}{\boldsymbol{\epsilon}}
\newcommand{\gsteperr}{\bar{\boldsymbol{\epsilon}}}
\newcommand{\rhserr}{\delta}
\newcommand{\rhsserr}{\boldsymbol{\delta}}

\newcommand{\bff}{\mathbf{f}}
\newcommand{\bFf}{\mathbf{F}}
\newcommand{\bfb}{\mathbf{f}_u}
\newcommand{\bfbt}{\tilde{\mathbf{f}}_u}
\newcommand{\btf}{\mathbf{\tilde{f}}}
\newcommand{\bone}{\mathbf{1}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bbh}{\hat{\mathbf{b}}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bt}{\mathbf{t}}
\newcommand{\bg}{\mathbf{g}}
\newcommand{\bfe}{\mathbf{e}}
\newcommand{\mC}{\m{C}}

\newcommand{\Rmin}{\overline{R}(\psi_1,\dots,\psi_k)}

\renewcommand{\v}[1]{\mathbf{#1}}


\newcommand\strutT{\rule{0pt}{2.6ex}}
\newcommand\strutB{\rule[-1.2ex]{0pt}{0pt}} 
\newcommand{\deltaset}{\bar{\boldsymbol{\delta}}}


